Nudging Nutrition: Lessons from the Danish "Fat Tax"

In October 2011, Denmark introduced the world's first and, to date, only tax targeting saturated fat. However, this tax was subsequently abolished in January 2013. Leveraging exogenous variation from untaxed Northern-German consumers, we employ a difference-in-differences approach to estimate the causal effects of both the implementation and repeal of the tax on consumption and expenditure behavior across eight product categories targeted by the tax. Our findings reveal significant heterogeneity in the tax's impact across these products. During the taxed period, there was a notable decline in consumption of bacon, liver sausage, and cheese, particularly among low-income households. In contrast, expenditure on butter, cream, and margarine increased as prices rose. Interestingly, we do not observe any difference in expenditure increases between high and low-income households, suggesting that the latter were disproportionately affected by the tax. After the repeal of the tax, we do not observe any significant decline in consumption. On the contrary, there was an overall increase in consumption for certain products, prompting concerns about unintended consequences resulting from the brief implementation of the tax. Finally, we find strong evidence on an overall increase purchases of butter abroad for households living less than 50 km from the German boarder but we do not find strong evidence of spatial heterogeneous effects of the tax.

==> results/abolishment.tex <==

% latex table generated in R 4.3.1 by xtable 1.8-4 package
% Tue Oct 17 11:00:43 2023
\begin{table}[tb]
\centering
\caption{The causal effect of the Danish fat tax on the average quarterly consumption and expenditure during the two years after abolishment of the tax (January 2013 to December 2014), using the final tax period (October 2012 to December 2012) as reference period.}
\label{tab:results_abolishment}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lcccccccc}
  \hline \hline
  & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) \\
 & Bacon & Butter & Cheese & Cream & Liver sausage & Margarine & Salami & Sour cream \\ [-0.5em]
  &  &  &  &  & and pat\'e &  &  &  \\ [0.5em]
  \hline
  \multicolumn{9}{l}{\textbf{Panel A: Quarterly average weight consumed in gr/ml}} \\ \hline
  \textit{Danish fat tax (ATT)} & $124.442^{**}$ & 5.298 & $557.856^{***}$ & -35.433 & $195.790^{***}$ & 72.082 & $131.118^{**}$ & 78.072 \\ 
  \textit{(se)} & (42.177) & (86.445) & (115.098) & (89.103) & (50.680) & (98.307) & (40.289) & (40.092) \\
  \textit{\% change} & 23.43\%  & 0.33\%  & 22.52\%  & -2.54\%  & 19.36\%  & 4.20\%  & 25.39\%  & 13.17\%  \\ 
  \textit{obs.} & 22,354 & 28,507 & 23,735 & 27,544 & 23,315 & 27,085 & 23,312 & 25,831 \\ 
  \textit{p-val. pre-trend} & 0.310 & 0.000 & 0.296 & 0.335 & 0.334 & 0.018 & 0.414 & 0.564 \\    \hline
  \multicolumn{9}{l}{\textbf{Panel B: Quarterly average expenditure in Euro cents}} \\ \hline 
  \textit{Danish fat tax (ATT)} & 57.635 & $-171.538^{***}$ & $415.404^{***}$ & -24.235 & $122.264^{**}$ & $-67.918^{**}$ & $136.449^{***}$ & 7.812 \\ 
  \textit{(se)} & (29.636) & (42.352) & (92.873) & (26.516) & (33.875) & (22.868) & (38.423) & (11.110) \\ 
  \textit{\% change} & 15.85\%  & -16.77\%  & 19.19\%  & -4.51\%  & 22.67\%  & -13.20\%  & 25.21\%  & 4.28\%  \\ 
  \textit{obs.} & 22,354 & 28,507 & 23,735 & 27,544 & 23,315 & 27,085 & 23,312 & 25,831 \\
  \textit{p-val. pre-trend} & 0.456 & 0.000 & 0.358 & 0.833 & 0.051 & 0.013 & 0.252 & 0.093 \\ 
      \hline
  \multicolumn{8}{l}{\textbf{Panel C: Quarterly average amount (in packages) consumed}} \\ \hline
  \textit{Danish fat tax (ATT)} & $0.430^{**}$ & -0.017 & $0.938^{*}$ & 0.145 & $0.782^{**}$ & 0.144 & $0.654^{**}$ & 0.341 \\ 
  \textit{(se)} & (0.158) & (0.340) & (0.393) & (0.327) & (0.255) & (0.187) & (0.234) & (0.175) \\ 
  \textit{\% change} & 21.53\%  & -0.26\%  & 21.14\%  & 4.47\%  & 26.19\%  & 3.87\%  & 23.69\%  & 26.58\%  \\  
  \textit{obs.} & 22,354 & 28,507 & 23,735 & 27,544 & 23,315 & 27,085 & 23,312 & 25,831 \\ 
  \textit{p-val. pre-trend} & 0.128 & 0.000 & 0.914 & 0.956 & 0.577 & 0.002 & 0.881 & 0.495 \\ 
   \hline \hline
   \multicolumn{9}{p{1.3\textwidth}}{\normalsize Significance level: * $p<0.1$ ** $p<0.05$ *** $p<0.01$. Standard errors clustered at unit level. \textit{\% change} compares the estimated tax average to the pre-tax sample mean for Danish households. The estimates are obtained using the doubly robust DID approach, controlling for age of head of household, number of children under 15, gender, ISCED, income level, and household size.}\\ 
\end{tabular}
\end{adjustbox}
\end{table}

\begin{table}[tb]
\centering
\caption{The causal effect of the Danish fat tax on the average quarterly consumption and expenditure during the two years after abolishment of the tax (January 2013 to December 2014), using the pre-tax period (January 2011 to March 2011) as reference period.}
\label{tab:results_abolishment_vs_pretax}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lcccccccc}
  \hline \hline
  & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) \\
 & Bacon & Butter & Cheese & Cream & Liver sausage & Margarine & Salami & Sour cream \\ [-0.5em]
  &  &  &  &  & and pat\'e &  &  &  \\ [0.5em]
  \hline
  \multicolumn{9}{l}{\textbf{Panel A: Quarterly average weight consumed in gr/ml}} \\ \hline
  \textit{Danish fat tax (ATT)} & 0.586 & $256.953^{**}$ & 31.182 & 117.048 & 1.505 & $325.944^{**}$ & 5.839 & $90.648^{*}$ \\ 
  \textit{(se)} & (35.004) & (72.408) & (129.746) & (71.148) & (46.676) & (92.464) & (37.856) & (35.617) \\ 
  \textit{\% change} & 0.10\% & 16.05\% & 1.15\% & 8.31\% & 0.14\% & 18.05\% & 1.05\% & 15.41\% \\ 
  \textit{obs.} & 33,510 & 45,295 & 36,043 & 43,648 & 35,160 & 42,954 & 35,175 & 40,299 \\ 
  \textit{p-val. pre-trend} & 0.182 & 0.362 & 0.268 & 0.369 & 0.859 & 0.853 & 0.959 & 0.138 \\ \hline
  \multicolumn{9}{l}{\textbf{Panel B: Quarterly average expenditure in Euro cents}} \\ \hline 
  \textit{Danish fat tax (ATT)} & 0.024 & $162.860^{***}$ & 12.967 & $57.764^{**}$ & -33.561 & 39.009 & 21.002 & $37.947^{**}$ \\ 
  \textit{(se)} & (26.678) & (38.977) & (105.804) & (19.152) & (30.410) & (21.705) & (38.239) & (10.451) \\ 
  \textit{\% change} & 0.01\% & 16.92\% & 0.56\% & 11.39\% & -5.73\% & 7.66\% & 3.59\% & 21.65\% \\ 
  \textit{obs.} & 33,510 & 45,295 & 36,043 & 43,648 & 35,160 & 42,954 & 35,175 & 40,299 \\ 
  \textit{p-val. pre-trend} & 0.516 & 0.000 & 0.235 & 0.668 & 0.950 & 0.734 & 0.905 & 0.050 \\ 
  \hline
  \multicolumn{8}{l}{\textbf{Panel C: Quarterly average amount (in packages) consumed}} \\ \hline
  \textit{Danish fat tax (ATT)} & 0.175 & $ 1.348^{***}$ & 0.586 & 0.058 & -0.001 & $ 0.916^{***}$ & $ 0.597^{*}$ & 0.285 \\ 
  \textit{(se)} & (0.150) & (0.294) & (0.368) & (0.254) & (0.196) & (0.210) & (0.222) & (0.145) \\ 
  \textit{\% change} & 8.53\% & 20.86\% & 12.83\% & 1.74\% & -0.04\% & 23.65\% & 21.17\% & 22.28\% \\ 
  \textit{obs.} & 33,510 & 45,295 & 36,043 & 43,648 & 35,160 & 42,954 & 35,175 & 40,299 \\ 
  \textit{p-val. pre-trend} & 0.982 & 0.472 & 0.282 & 0.939 & 0.991 & 0.797 & 0.989 & 0.481 \\ 
   \hline \hline
   \multicolumn{9}{p{1.3\textwidth}}{\normalsize Significance level: * $p<0.1$ ** $p<0.05$ *** $p<0.01$. Standard errors clustered at unit level. \textit{\% change} compares the estimated tax average to the pre-tax sample mean for Danish households. The estimates are obtained using the doubly robust DID approach, controlling for age of head of household, number of children under 15, gender, ISCED, income level, and household size.}\\ 
\end{tabular}
\end{adjustbox}
\end{table}

==> results/heterogeneity_plots.tex <==

\begin{figure}[htbp] 
  \centering
  \begin{subfigure}{\textwidth}
    \centering
    \includegraphics[width=0.825\textwidth]{figures/low_high_income_comparison/income_barplot_weight.jpg} 
    \caption{Average quarterly weight consumed (gr/ml).}
    \label{fig:low_high_income_weight}
  \end{subfigure}
  \hfill
  \begin{subfigure}{\textwidth}
    \centering
    \includegraphics[width=0.825\textwidth]{figures/low_high_income_comparison/income_barplot_expenditure.jpg}
    \caption{Average quarterly expenditure in Euro cents.}
    \label{fig:low_high_income_expenditure}
  \end{subfigure}
  \hfill
  \begin{subfigure}{\textwidth}
    \centering
    \includegraphics[width=0.825\textwidth]{figures/low_high_income_comparison/income_barplot_amount.jpg} 
    \caption{Average quarterly number of packages.}
    \label{fig:low_high_income_amount}
  \end{subfigure}
  \caption{Doubly robust DID estimates of the causal effect of the Danish fat tax during the tax period (October 2011 to December 2012), subgrouping for low and high income households and controlling for household characteristics. Low-income households are defined as households with very low income or low income. High-income households are defined as households with very high income or high income.  95\% confidence intervals indicated in dark red. }
  \label{fig:low_high_income}
\end{figure}






==> results/main_table.tex <==

% latex table generated in R 4.3.1 by xtable 1.8-4 package
% Mon Oct 16 15:30:44 2023
\begin{table}[tb]
\centering
\caption{The causal effect of the Danish fat tax on the average quarterly consumption and expenditure during the tax period (October 2011 to December 2012).}
\label{tab:main_results}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lcccccccc}
  \hline \hline
  & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) \\
 & Bacon & Butter & Cheese & Cream & Liver sausage & Margarine & Salami & Sour cream \\ [-0.5em]
  &  &  &  &  & and pat\'e &  &  &  \\ [0.5em]
  \hline
  \multicolumn{9}{l}{\textbf{Panel A: Quarterly average weight consumed in gr/ml}} \\ \hline
  
  \textit{Danish fat tax (ATT)} & $-56.891$ & 73.292 & $-351.109^{*}$ & 27.663 & $-120.925^{*}$ & 114.433 & $-66.774^{**}$ & 27.768 \\ 
  \textit{(se)} & (35.788) & (78.927) & (127.263) & (65.761) & (47.718) & (101.072) & (36.823) & (36.351) \\ 
  \textit{\% change} & -10.07\% & 4.81\% & -13.05\% & 2.01\% & -11.07\% & 6.24\% & -12.10\% & 4.85\% \\ 
  \textit{obs.} & 29,645 & 40,929 & 32,129 & 39,274 & 31,246 & 38,687 & 31,243 & 36,121 \\ 
  \textit{p-val. pre-trend} & 0.273 & 0.384 & 0.344 & 0.455 & 0.846 & 0.772 & 0.963 & 0.208 \\ 
    \hline
  \multicolumn{9}{l}{\textbf{Panel B: Quarterly average expenditure in Euro cents}} \\ \hline
  \textit{Danish fat tax (ATT)} & -25.075 & $234.879^{***}$ & $-240.166$ & $70.823^{**}$ & $-81.437^{*}$ & $84.643^{***}$ & $-50.452$ & $27.131^{*}$ \\ 
  \textit{(se)} & (26.216) & (37.992) & (105.520) & (19.589) & (28.147) & (22.041) & (38.160) & (10.413) \\ 
  \textit{\% change} & -6.85\% & 25.20\% & -10.42\% & 14.49\% & -13.75\% & 15.42\% & -8.81\% & 16.03\% \\ 
  \textit{obs.} & 29,645 & 40,929 & 32,129 & 39,274 & 31,246 & 38,687 & 31,243 & 36,121 \\ 
  \textit{p-val. pre-trend} & 0.653 & 0.000 & 0.505 & 0.748 & 0.929 & 0.603 & 0.921 & 0.075 \\ 
    \hline
  \multicolumn{8}{l}{\textbf{Panel C: Quarterly average amount (in packages) consumed}} \\ \hline
  \textit{Danish fat tax (ATT)} & -0.010 & 0.361 & -0.304 & -0.202 & $-0.463$ & $0.404$ & -0.009 & 0.059 \\ 
  \textit{(se)} & (0.160) & (0.314) & (0.398) & (0.272) & (0.199) & (0.198) & (0.233) & (0.145) \\ 
  \textit{\% change} & -0.51\% & 6.01\% & -7.09\% & -6.19\% & -14.40\% & 10.39\% & -0.33\% & 4.77\% \\ 
  \textit{obs.} & 29,645 & 40,929 & 32,129 & 39,274 & 31,246 & 38,687 & 31,243 & 36,121 \\ 
  \textit{p-val. pre-trend} & 0.987 & 0.557 & 0.249 & 0.954 & 0.984 & 0.795 & 0.977 & 0.512 \\ 
   \hline \hline
   \multicolumn{9}{p{1.3\textwidth}}{\normalsize Significance level: * $p<0.1$ ** $p<0.05$ *** $p<0.01$. Standard errors clustered at unit level. \textit{\% change} compares the estimated tax average to the pre-tax sample mean for Danish households. The estimates are obtained using the doubly robust DID approach, controlling for age of head of household, number of children under 15, gender, ISCED, income level, and household size.}\\ 
\end{tabular}
\end{adjustbox}
\end{table}



==> results/price_mechanism_abolishment.tex <==

% latex table generated in R 4.3.0 by xtable 1.8-4 package
% Mon Jul 31 13:24:19 2023
\begin{table}[!htb]
\centering
\caption{The causal effect of the Danish fat tax on quarterly average price during the two years after the tax was abolished (January 2013 to December 2014), using the final tax period (October 2012 to December 2012) as reference period.}
\label{tab:mechanism_abolishment}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lcccccccc}
  \hline \hline
  & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) \\
 & Bacon & Butter & Cheese & Cream & Liver sausage & Margarine & Salami & Sour cream \\ [-0.5em]
  &  &  &  &  & and pat\'e &  &  &  \\ [0.5em]
  \hline
\textit{Danish fat tax (ATT)} & -3.444 & $-10.671^{***}$ & -2.434 & $-1.701^{***}$ & -3.917 & $-4.054^{***}$ & -3.465 & $-1.898^{***}$ \\ 
  \textit{(se)} & (2.894) & (0.676) & (1.996) & (0.474) & (2.716) & (0.569) & (3.595) & (0.530) \\ 
  \textit{\% change} & -4.82\%  & -15.79\%  & -2.58\%  & -4.18\%  & -6.27\%  & -13.03\%  & -2.92\%  & -5.83\%  \\ 
  \textit{obs.} & 12,568 & 22,942 & 19,930 & 19,452 & 16,170 & 19,230 & 15,208 & 13,678 \\ 
  \textit{p-val. pre-trend} & 0.787 & 0.000 & 0.489 & 0.000 & 0.538 & 0.032 & 0.533 & 0.000 \\ 
   \hline \hline
   \multicolumn{9}{p{1.3\textwidth}}{\normalsize Significance level: * $p<0.1$ ** $p<0.05$ *** $p<0.01$. Standard errors clustered at unit level. \textit{\% change} compares the estimated tax average to the pre-tax sample mean for Danish households. The estimates are obtained using the doubly robust DID approach.}\\ 
\end{tabular}
\end{adjustbox}
\end{table}

\begin{table}[!htb]
\centering
\caption{The causal effect of the Danish fat tax on quarterly average price during the two years after the tax was abolished (January 2013 to December 2014), using the pre-tax period (January 2011 to March 2011) as reference period.}
\label{tab:mechanism_abolishment_vs_pretax}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lcccccccc}
  \hline \hline
  & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) \\
 & Bacon & Butter & Cheese & Cream & Liver sausage & Margarine & Salami & Sour cream \\ [-0.5em]
  &  &  &  &  & and pat\'e &  &  &  \\ [0.5em]
  \hline
\textit{Danish fat tax (ATT)} & -6.734 & $2.039^{**}$ & 0.086 & -0.093 & $-11.091^{***}$ & $-1.483^{**}$ & -5.631 & $2.585^{***}$ \\ 
  \textit{(se)} & (2.889) & (0.583) & (1.644) & (0.371) & (2.414) & (0.484) & (3.351) & (0.572) \\ 
  \textit{\% change} & -9.67\% & 3.22\% & 0.09\% & -0.24\% & -17.95\% & -5.01\% & -4.73\% & 8.15\% \\ 
  \textit{obs.} & 19,235 & 36,058 & 31,104 & 30,979 & 25,609 & 31,466 & 23,729 & 21,739 \\ 
  \textit{p-val. pre-trend} & 0.723 & 0.000 & 0.757 & 0.009 & 0.615 & 0.557 & 0.820 & 0.000 \\ 
   \hline \hline
   \multicolumn{9}{p{1.3\textwidth}}{\normalsize Significance level: * $p<0.1$ ** $p<0.05$ *** $p<0.01$. Standard errors clustered at unit level. \textit{\% change} compares the estimated tax average to the pre-tax sample mean for Danish households. The estimates are obtained using the doubly robust DID approach.}\\ 
\end{tabular}
\end{adjustbox}
\end{table}

==> results/price_mechanism_graphs.tex <==
\FloatBarrier

\begin{figure}[htbp]
    \centering
    
    \begin{minipage}{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/unbalanced_2009_2014_anticipationTRUE/unbalanced_price_Bacon_2009_2014_2011_75_TRUE.JPG}
        \caption{Bacon.}
        \label{fig:evolution_price_bacon}
    \end{minipage}
    \hfill
    \begin{minipage}{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/unbalanced_2009_2014_anticipationTRUE/unbalanced_price_Butter_2009_2014_2011_75_TRUE.JPG}
        \caption{Butter.}
        \label{fig:evolution_price_butter}
    \end{minipage}
    
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/unbalanced_2009_2014_anticipationTRUE/unbalanced_price_Cheese_2009_2014_2011_75_TRUE.JPG}
        \caption{Cheese.}
        \label{fig:evolution_price_cheese}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/unbalanced_2009_2014_anticipationTRUE/unbalanced_price_Cream_2009_2014_2011_75_TRUE.JPG}
        \caption{Cream.}
        \label{fig:evolution_price_cream}
    \end{minipage}

    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/unbalanced_2009_2014_anticipationTRUE/unbalanced_price_Liver_sausage_and_pate_2009_2014_2011_75_TRUE.JPG}
        \caption{Liver sausage and pat\'e.}
        \label{fig:evolution_price_liver}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/unbalanced_2009_2014_anticipationTRUE/unbalanced_price_Margarine_2009_2014_2011_75_TRUE.JPG}
        \caption{Margarine.}
        \label{fig:evolution_price_margarine}
    \end{minipage}

        \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/unbalanced_2009_2014_anticipationTRUE/unbalanced_price_Salami_2009_2014_2011_75_TRUE.JPG}
        \caption{Salami.}
        \label{fig:evolution_price_salami}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/unbalanced_2009_2014_anticipationTRUE/unbalanced_price_Sour_cream_2009_2014_2011_75_TRUE.JPG}
        \caption{Sour cream.}
        \label{fig:evolution_price_Sour_cream}
    \end{minipage}
    
    
    \caption{Price time average treatment effects, $ATT(q)$. The two vertical dashed lines indicate the introduction and abolishment of the Danish fat tax, respectively. Red estimates of effect on average quarterly price in Euro cents. and simultaneous 95\% confidence intervals for pre-tax periods and blue estimates for tax-period estimates, clustered at unit level. Under parallel trends, red estimates should be close to zero.}
    \label{fig:price_mechanism_graphs}
\end{figure}

\clearpage

==> results/price_mechanism_table.tex <==

\begin{table}[!bt]
\centering
\caption{The causal effect of the Danish fat tax on quarterly average price paid per 100 units during the tax period (October 2011 to December 2012).}
\label{tab:results_price_mechanism}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lcccccccc}
  \hline \hline
  & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) \\
 & Bacon & Butter & Cheese & Cream & Liver sausage & Margarine & Salami & Sour cream \\ [-0.5em]
  &  &  &  &  & and pat\'e &  &  &  \\ [0.5em]
  \hline
\textit{Danish fat tax (ATT)} & -1.918 & $14.935^{***}$ & $3.610$ & $3.968^{***}$ & -3.076 & $3.566^{***}$ & 1.976 & $3.863^{***}$ \\ 
  \textit{(se)} & (2.916) & (0.558) & (1.660) & (0.408) & (2.478) & (0.509) & (3.292) & (0.586) \\ 
  \textit{\% change} & -2.81\% & 23.44\% & 3.92\% & 10.58\% & -4.95\% & 11.35\% & 1.65\% & 12.31\% \\ 
  \textit{obs.} & 16,863 & 32,189 & 27,511 & 27,735 & 22,726 & 28,682 & 20,925 & 19,590 \\ 
  \textit{p-val. pre-trend} & 0.554 & 0.000 & 0.683 & 0.009 & 0.718 & 0.441 & 0.833 & 0.000 \\ 
   \hline \hline
   \multicolumn{9}{p{1.3\textwidth}}{\normalsize Significance level: * $p<0.1$ ** $p<0.05$ *** $p<0.01$. Standard errors clustered at unit level. \textit{\% change} compares the estimated tax average to the pre-tax sample mean for Danish households. The estimates are obtained using the doubly robust DID approach.}\\ 
\end{tabular}
\end{adjustbox}
\end{table}



